Avoiding Scalability Collapse by Restricting Concurrency

Saturated locks often degrade the performance of a multithreaded application, leading to a so-called scalability collapse problem. This problem arises when a growing number of threads circulating through a saturated lock causes the overall application performance to fade or even drop abruptly. This problem is particularly (but not solely) acute on oversubscribed systems (systems with more threads than available hardware cores). In this paper, we introduce GCR (generic concurrency restriction), a mechanism that aims to avoid the scalability collapse. GCR, designed as a generic, lock-agnostic wrapper, intercepts lock acquisition calls, and decides when threads would be allowed to proceed with the acquisition of the underlying lock. Furthermore, we present GCR-NUMA, a non-uniform memory access (NUMA)-aware extension of GCR, that strives to ensure that threads allowed to acquire the lock are those that run on the same socket. The extensive evaluation that includes more than two dozen locks, three machines and three benchmarks shows that GCR brings substantial speedup (in many cases, up to three orders of magnitude) in case of contention and growing thread counts, while introducing nearly negligible slowdown when the underlying lock is not contended. GCR-NUMA brings even larger performance gains starting at even lighter lock contention.

==> macros.tex <==
\newcommand{\remove}[1] {}
%\newcommand{\remove}[1] {#1}

%\newcommand{\comment}[1]{}
\newcommand{\comment}[1]{\textbf{#1}}
\newcommand{\alex}[1]{\comment{[Alex] #1}}

\newcommand{\hafc} {\texttt{HCF}}

\newcommand{\p} {~phase}

\newcommand{\pc}[1]{\lstinline{#1}}
